Time-Dependent 2-D Vector Field Topology: An Approach Inspired by Lagrangian Coherent Structures

This paper presents an approach to a time-dependent variant of the concept of vector field topology for 2-D vector fields. Vector field topology is defined for steady vector fields and aims at discriminating the domain of a vector field into regions of qualitatively different behaviour. The presented approach represents a generalization for saddle-type critical points and their separatrices to unsteady vector fields based on generalized streak lines, with the classical vector field topology as its special case for steady vector fields. The concept is closely related to that of Lagrangian coherent structures obtained as ridges in the finite-time Lyapunov exponent field. The proposed approach is evaluated on both 2-D time-dependent synthetic and vector fields from computational fluid dynamics.

==> Makefile <==
CC1 = latex
CC2 = bibtex
CC3 = dvips
CC4 = ps2pdf

FORMAT = a4

# Main file name
SRC = timeVFT


TEX_FILE = $(SRC).tex

DVI = $(SRC).dvi
PS = $(SRC).ps
PDF = $(SRC).pdf

default: latexing3 ps2pdfs

# Latexing the main tex file
latexing1: $(TEX_FILE)
	$(CC1) $(TEX_FILE)

# Bibtexing the included files
bibtexing: latexing1
	$(CC2) $(SRC) 

# Then latexing once 
latexing2: bibtexing
	$(CC1) $(TEX_FILE)

# Then latexing twice 
latexing3: latexing2 
	$(CC1) $(TEX_FILE)

dvi2ps: latexing3
#	$(CC3) -t $(FORMAT) -Ppdf -G0 -Pdownload35 -o $(PS) $(DVI)
	$(CC3) -t $(FORMAT) -Ppdf -G0 -o $(PS) $(DVI)

ps2pdfs: dvi2ps
#	$(CC4) -sPAPERSIZE=$(FORMAT) -dMaxSubsetPct=100 -dCompatibilityLevel=1.3 \
#		-dSubsetFonts=true -dEmbedAllFonts=true -dMaxSubsetPct=100 \
#		-dAutoFilterColorImages=false \
#		-dAutoFilterGrayImages=false \
#		-dColorImageFilter=/FlateEncode \
#		-dGrayImageFilter=/FlateEncode \
#		-dMonoImageFilter=/FlateEncode -dPDFSETTINGS=/prepress $(PS) $(PDF)
# this version is for GhostScript 8.x according to EuroVis
	$(CC4) -dPDFSETTINGS=/prepress \
	-dCompatibilityLevel=1.3 \
	-dAutoFilterColorImages=false \
	-dAutoFilterGrayImages=false \
	-dColorImageFilter=/FlateEncode \
	-dGrayImageFilter=/FlateEncode \
	-dMonoImageFilter=/FlateEncode \
	-dDownsampleColorImages=false \
	-dDownsampleGrayImages=false $(PS) $(PDF)
	rm -f *.ps

pdf: ps2pdfs

ps: dvi2ps

sdvi2ps: latexing1
#	$(CC3) -t $(FORMAT) -Ppdf -G0 -Pdownload35 -o $(PS) $(DVI)
	$(CC3) -t $(FORMAT) -Ppdf -G0 -o $(PS) $(DVI)

sps2pdfs: sdvi2ps
#	$(CC4) -sPAPERSIZE=$(FORMAT) -dMaxSubsetPct=100 -dCompatibilityLevel=1.3 \
#	       -dSubsetFonts=true -dEmbedAllFonts=true -dMaxSubsetPct=100 \
#	       -dAutoFilterColorImages=false \
#	       -dAutoFilterGrayImages=false \
#	       -dColorImageFilter=/FlateEncode \
#	       -dGrayImageFilter=/FlateEncode \
#	       -dMonoImageFilter=/FlateEncode -dPDFSETTINGS=/prepress $(PS) $(PDF)
# this version is for GhostScript 8.x according to EuroVis
	$(CC4) -dPDFSETTINGS=/prepress \
	-dCompatibilityLevel=1.3 \
	-dAutoFilterColorImages=false \
	-dAutoFilterGrayImages=false \
	-dColorImageFilter=/FlateEncode \
	-dGrayImageFilter=/FlateEncode \
	-dMonoImageFilter=/FlateEncode \
	-dDownsampleColorImages=false \
	-dDownsampleGrayImages=false $(PS) $(PDF)

nobibtex: sps2pdfs

clean: 
	-rm -f *.aux *.bbl *.blg *.dvi *.err *.hp *.lof *.log *.lot *.toc *.lbl *.ps *.pdf

